A Review on Communication Protocols for Autonomous Unmanned Aerial Vehicles for Inspection Application

The communication system is a critical part of the system design for the autonomous UAV. It has to address different considerations, including efficiency, reliability and mobility of the UAV. In addition, a multi-UAV system requires a communication system to assist information sharing, task allocation and collaboration in a team of UAVs. In this paper, we review communication solutions for supporting a team of UAVs while considering an application in the power line inspection industry. We provide a review of candidate wireless communication technologies {for supporting communication in UAV applications. Performance measurements and UAV-related channel modeling of those candidate technologies are reviewed. A discussion of current technologies for building UAV mesh networks is presented. We then analyze the structure, interface and performance of robotic communication middleware, ROS and ROS2. Based on our review, the features and dependencies of candidate solutions in each layer of the communication system are presented.

==> src/tables.tex <==
\begin{table}[]
\centering
\scriptsize
\caption{ {Communication types and characteristics.}}
\begin{tabular}{|l|l|l|l|l|l|}
\hline
\multicolumn{1}{|c|}{\textbf{Category}}                                        & \multicolumn{1}{c|}{\textbf{Use Case}}                               & \multicolumn{1}{c|}{\textbf{Flow Type}}                              & \textbf{Priority} & \textbf{\begin{tabular}[c]{@{}l@{}}Data Size\\ (Kbyte)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Mobility\\(m/s)\end{tabular}}                                               \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Data \\ Exchange\end{tabular}}      & \begin{tabular}[c]{@{}l@{}}Upload\\ Mission Data\end{tabular}     & Unicast                                                         & Low               & $>1000$                                                           & \begin{tabular}[c]{@{}l@{}}Static or \\ $<1$\end{tabular} \\ \cline{2-6} 
                                                                               & \begin{tabular}[c]{@{}l@{}}Send\\ Environment\\ Data\end{tabular} & Unicast                                                         & Low               & $>1000$                                                          & \begin{tabular}[c]{@{}l@{}}Static or \\ $<1$\end{tabular} \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Command \\ \& Control\end{tabular}} & \begin{tabular}[c]{@{}l@{}}Send \\ Command\end{tabular}           & Unicast                                                         & High              & $<0.1$                                                           & $1 - 10$       \\ \cline{2-6} 
                                                                               & Report Status                                                     & Unicast                                                         & Low               & $<0.1$                                                          &  $1 - 10$        \\ \hline
\multirow{2}{*}{Clustering}                                                    & \begin{tabular}[c]{@{}l@{}}Manage \\ Connectivity\end{tabular}    & \begin{tabular}[c]{@{}l@{}}Multicast \\ \& Unicast\end{tabular} & Middle            & $<0.1$                                                           &  $1 - 10$        \\ \cline{2-6} 
                                                                               & Share Info                                                        & Unicast                                                         & Low               & \begin{tabular}[c]{@{}l@{}}$<100$ \end{tabular}      &  $1 - 10$        \\ \hline
\end{tabular}
\label{Tab:message_profile}
\end{table}



\begin{table}[]
\centering
\caption{Wireless technologies for UAV applications: In-field measurements.}
\label{table:In_field_measurements}
\begin{threeparttable}

\begin{tabular}{|>{\centering}p{0.14\textwidth}|>{\centering}p{0.17\textwidth}|>{\centering}p{0.12\textwidth}|>{\centering}p{0.18\textwidth}|>{\centering}p{0.09\textwidth}|>{\centering}p{0.08\textwidth}|}
\hline 
\textbf{Network Type} & \textbf{Technology} & \textbf{Link Type} & \textbf{Throughput (Mbps)} & \textbf{Range (m)} & \textbf{Refs.}\tabularnewline
\hline 
\multirow{4}{0.09\textwidth}{Cellular} & 3G & A2G, G2A & 0.384 & 100 & \cite{Zhu2015}\tabularnewline
\cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6} 
 & LTE & A2G, G2A & 0.1-18.5 & 20-4500 & \cite{LTEAmorim2017} \cite{LTEKovacs2018} \cite{LTE2Kovacs2018} \cite{QualcommTechnologies2017} \tabularnewline
%\cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6} 
% & LTE & A2G, G2A & 0.1-0.48 & 1000-4500 & \cite{LTE2Kovacs2018}\cite{QualcommTechnologies2017}\tabularnewline
%\cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6} 
% & LTE & A2G & 18.5 & 20 & \cite{LTE2Kovacs2018}\tabularnewline
%\cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6} 
% & LTE & A2G, G2A & 0.48 & 1000 & \cite{QualcommTechnologies2017}\tabularnewline
\cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6} 
 & LTE-M & Drive test & 0.1 & 15000 & \cite{Lauridsen2016}\tabularnewline
\cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6} 
 & NB-IoT & Drive test & 0.2 & 15000 & \cite{Lauridsen2016}\tabularnewline
\hline
\multirow{6}{0.09\textwidth}{WLAN} %& 802.15.4 & A2G, A2A & 0.056 & 500 & \cite{Allred2007}\tabularnewline
% & 802.15.4 & A2G & 0.250 & 1500 & \cite{Asadpour2013}\tabularnewline
%\cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6} 
 %& 802.15.4 & A2G, A2A & 0.056 & 500 & \cite{Allred2007}\tabularnewline
%\cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6} 
 & 802.11b & A2G & 1.2 & 2000 & \cite{Brown}\tabularnewline
\cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6} 
 & 802.11a & A2G, G2A, A2A & 8-14 & 300-{500} & \cite{Yanmaz2013} \cite{ExperimentalYanmaz2014}
  {\cite{6953010}}\tabularnewline
\cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6} 
 & 802.11n & A2A & 2.2-20 & 80-300 & \cite{Asadpour2013} \cite{FromGroundAsadpour2013}\tabularnewline
%\cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6} 
% & 802.11n & A2A & 2.2 & 300 & \cite{FromGroundAsadpour2013}\tabularnewline
\cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6} 
 & 802.11g & G2A, A2G, A2A & 8 & 75 & \cite{Morgenthaler2012}\tabularnewline
%\cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6} 
% & 802.11a + 802.11s & G2A, A2G, A2A & 8 & 300 & \cite{ExperimentalYanmaz2014}\tabularnewline
\cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6} 
 & 802.11p & V2V & 3 & 400 & \cite{Lv2016}\tabularnewline
\cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6} 
 & 802.11ah & Outdoor moving & 0.15 & 300 & \cite{outdoorBellekens2017}\tabularnewline
\hline 
\multirow{3}{0.09\textwidth}{WPAN} & 802.15.4 & A2G, A2A & 0.056-0.250 & 500-1500 & \cite{Allred2007}\cite{Asadpour2013}\tabularnewline
  %& \textcolor{red}{UWB} &   &   &   & \tabularnewline 
%\cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6} 
% & \textcolor{red}{UWB} &   &   &   &  \tabularnewline
\hline
\multirow{2}{0.09\textwidth}{LPWAN} & LoRa 868 MHz, 915 MHz & Drive test & 0.006 & 650-1600 & \cite{loraAugustin2016}\cite{Rahmadhani2018}\tabularnewline
%\cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6} 
% & LoRa & A2G & 0.006 & 1600 & \cite{Rahmadhani2018}\tabularnewline
 \cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6} 
% & \textcolor{red}{LoRa 2.4 GHz} &  &  &  &  \textcolor{red}{\cite{XXX}}\tabularnewline
\hline
\end{tabular}
\begin{tablenotes}
	\item V2V: Vehicle to Vehicle (on ground) communication
	\item Drive test: The testbed is placed on a car to test the communication performance when driving on the road with different speed.
% 	\textcolor{red}{Put the references as [1, 2, 3-5,8] instead of the current format, [RHJ] but check with the style guide of MICPRO first.}
\end{tablenotes}
\end{threeparttable}
\end{table}

\begin{table}[h!]
\footnotesize
\caption{Surveyed Networking Protocols}

\begin{tabular}{|>{\raggedright}p{0.20\columnwidth}|>{\raggedright}p{0.18\columnwidth}|>{\raggedright}p{0.16\columnwidth}|>{\raggedright}p{0.20\columnwidth}|>{\raggedright}p{0.10\columnwidth}|}
\hline 
\textbf{Protocol} & \textbf{Type} & \textbf{Reactiveness} & \textbf{Metrics} & \textbf{Refs.} \tabularnewline
\hline 
HWMP (802.11s) & Hybrid & Hybrid & Range, PSR, Delay, Overhead & \cite{6477825,6953010,6125375,7980778} \tabularnewline
\hline 
BATMAN(-adv) & Link State & Proactive & Goodput, Delay & \cite{6125375} \tabularnewline
\hline 
OLSR & Link State & Proactive & Goodput, Delay &  \cite{6125375} \tabularnewline
\hline 
AODV & Distance Vector & Reactive & PSR, Goodput & \cite{hernandezmarcano2020} \tabularnewline
%\hline 
%ZRP & Hybrid & & [] \tabularnewline
\hline 
\end{tabular}
\label{table:meshtable}
\end{table}



\begin{table}[b]
\small
\caption{Concept mapping between ROS2 and DDS middleware}
\begin{tabular}{|c|c|c|}
\hline 
\multirow{2}{*}{\textbf{ROS2}} & \multicolumn{2}{c|}{\textbf{DDS middleware (FastRTPS)}}\tabularnewline
\cline{2-3} \cline{3-3} 
 & \textbf{Publisher-Subscriber layer} & \textbf{Writer-Reader layer}\tabularnewline
\hline 
Node & Participant & RTPSParticipant\tabularnewline
\hline 
Publisher & Publisher & RTPSWriter\tabularnewline
\hline 
Subscriber & Subscriber & RTPSReader\tabularnewline
\hline 
Service & Publisher + Subscriber & RTPSWriter + RTPSReader\tabularnewline
\hline 
Client & Publisher + Subscriber & RTPSWriter + RTPSReader\tabularnewline
\hline 
\end{tabular}
\label{table:concept-mapping}
\end{table}


\begin{table}[h!]
\footnotesize
\caption{Comparison of Advantages and Disadvantages in different ROS networks}

\begin{tabular}{|>{\raggedright}p{0.15\columnwidth}|>{\raggedright}p{0.39\columnwidth}|>{\raggedright}p{0.39\columnwidth}|}
\hline 
\textbf{Network} & \textbf{Advantages} & \textbf{Disadvantages}\tabularnewline
\hline 
Single-master ROS network & - Simple system structure

- Seamless integration with large amount of third-party software (ROS
package) fordifferent robotic functions & - Depends on a centralized device

- Very limited network scalability

- Limited extendability of ROS communication middleware with closely
coupled structure

- Cumbersome network configuration by default

- Not support discovery in networkby default

- Limited options to control communication QoS\tabularnewline
\hline 
Multi-master ROS network & - Relax the dependence on a centralized device

- Seamless integration with large amount of third-party software (ROS
package) for different robotic functions

- Improved network configuration process with the support of third-party
ROS packages

- Support discovery in network by third-party ROS packages & - Limited network scalability

- Limited extendability of ROS communication middleware with closely
coupled structure

- Limited options to control communication QoS\tabularnewline
\hline 
ROS2 network & - Flexible network topology

- Good network scalability

- Good extendability of ROS2 communication middleware with hierarchical
architecture

- Simple network configuration

- Support discovery in network

- Support reliable communication on top of UDP

- More options to control communication QoS & - Lack of third-party ROS2 packages

- Extra time cost for message conversion to fit DDS requirements\tabularnewline
\hline 
\end{tabular}
\label{table:proscons}
\end{table}



